Generating Visual Stories with Grounded and Coreferent Characters

Characters are important in narratives. They move the plot forward, create emotional connections, and embody the story's themes. Visual storytelling methods focus more on the plot and events relating to it, without building the narrative around specific characters. As a result, the generated stories feel generic, with character mentions being absent, vague, or incorrect. To mitigate these issues, we introduce the new task of character-centric story generation and present the first model capable of predicting visual stories with consistently grounded and coreferent character mentions. Our model is finetuned on a new dataset which we build on top of the widely used VIST benchmark. Specifically, we develop an automated pipeline to enrich VIST with visual and textual character coreference chains. We also propose new evaluation metrics to measure the richness of characters and coreference in stories. Experimental results show that our model generates stories with recurring characters which are consistent and coreferent to larger extent compared to baselines and state-of-the-art systems.

==> sec/dataset_creation.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/data_example.pdf}
%     \caption{An example from our \textit{CRAN} dataset, showcasing detailed character annotations within visual stories, along with quality labels. Character mentions are underlined in the story text. Identical characters are color-coded in images and story text, and visual/textual coreference chains are aligned with consistent character labels.}
%     \label{fig:data_example}
% \end{figure*}




\section{Dataset Creation}
\label{sec:dataset_creation}

\begin{table}[]
\centering
\resizebox{.48\textwidth}{!}{%
\begin{tabular}{lccrrr}
\hline
Dataset & Auto. & Coref. & \#Stories & \#Chars & \#Boxes \\
\hline
VIST-Char & \textcolor{red}{\usym{2717}} & \textcolor{ForestGreen}{\usym{2713}} & 0.7K & 3K & 5K \\
VWP & \textcolor{red}{\usym{2717}} & \textcolor{red}{\usym{2717}} & 12K & 157K & 157K \\
\textbf{CRAN (Ours)} & \textcolor{ForestGreen}{\usym{2713}} & \textcolor{ForestGreen}{\usym{2713}} & \textbf{40K} & \textbf{300K} & \textbf{520K}\\
\hline
\end{tabular}%
}
\caption{Comparison of statistics for datasets with character annotations. `Auto' indicates whether the dataset is annotated automatically. '\#stories' and '\#chars' refer to the number of visual stories and unique characters.}
\label{tab:stat}
\end{table}

To fine-tune \textsc{Otter-llama-7B} for the visually grounded story generation task, we developed an automated pipeline to create \textsc{CRAN}, a large-scale character dataset comprising 40K visual stories. This dataset provides detailed character annotations, including fine-grained character labels in images and aligned multimodal character coreference chains. The resulting dataset contains 300K unique characters, each associated with segmentation masks across images and a textual coreference chain, amounting to a total of 520K character appearances. To our knowledge, this is the first character-centric dataset of this scale generated entirely through an automated annotation pipeline. The statistics of \textsc{CRAN} and comparisons to previous character datasets are shown in Table~\ref{tab:stat}.

\subsection{Automatic Pipeline}
We propose an automated pipeline to perform such annotations.
This process includes three subtasks:
1) Visual character co-reference, which is to detect all the characters in the image sequence and identify characters into visual co-reference chains, i.e., which characters are the same person, 2) Textual character co-reference, which involves detecting character mentions and identify the co-reference chains in the story text, and 3) Multimodal alignment, which is to align the textual and visual co-reference chains to obtain multi-modal co-reference chains.
Next, we introduce our model for each task respectively.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/coref_in_one.pdf}
    \caption{Illustration of the proposed sequential character matching method and prompts used in textual character coreference resolution. (a) Character detections in the current Image$_{k+1}$, are compared for similarity against character clusters from the previous $k$ images to generate a similarity matrix. The best matches are then identified, and the matched character detections are added to the corresponding clusters. Detections that do not match any existing clusters are grouped into new clusters. (b) First, a QA-based prompting method is used to detect if each entity and noun chunk in the story refers to characters. Then, we designed a structured prompt template, which can handle both single and plural characters, allowing the LLM to produce character clusters.}
    \label{fig:coref_in_one}
\end{figure*}


\subsubsection{Visual Character Co-reference}
\label{sec:visual_coref}
% Previous visual coreference methods \cite{schroff2015facenet,liu2023detecting} rely on clustering algorithms, but they have three major drawbacks: 1) they depend on facial features, which often fail to detect side-view faces, which are common in visual stories; 2) they require a predefined number of clusters, which is unknown from the input images; and
% % 3) they ignore the fact that characters appearing in the same image cannot be the same person.
% 3) they often incorrectly identifies different characters in the same image as the same person.
% To address these issues, we propose a Sequential Character Matching algorithm (shown in Figure \ref{fig:coref_in_one}a) that effectively corrects these incorrect assumptions, achieving state-of-the-art results.
The task is to detect character bounding boxes from an image sequence and then identify which detections represent the same character, thereby constructing visual coreference chains.
Previous methods typically cluster the features of bounding boxes directly into clusters.
In contrast, our work proposes a Sequential Character Matching method (shown in Figure \ref{fig:coref_in_one}a) to overcome the limitations of clustering-based approaches (see Section \ref{vcoref-related_work} for a detailed discussion of comparisons).
\paragraph{Sequential Character Matching}
For the input image sequence, we first apply a pretrained object detector and retain detections with the label \textit{Person}, a confidence score higher than 0.9, and covering at least 10\% of the image area to remove background characters.
The construction of our visual coreference chain is iterative: first, all the characters detected in the first image are regarded as new characters and added to the chain.
Subsequently, for every character detection in image$_{k+1}$, we compute the pairwise matching score between it and every existing character cluster from previous images$_{0:k}$, and obtain a similarity matrix.
We employ the embeddings from pretrained image encoder
% from pretrained CLIP ~\cite{radford2021learning,ilharco_gabriel_2021_5143773}
to measure the similarity between two character crops.
We model this as a Bipartite Graph Matching problem and apply the Kuhn-Munkres algorithm \cite{kuhn1955hungarian} to the similarity matrix and obtain the matching results.
We added a threshold condition to the Kuhn-Munkres algorithm.
This means not all current characters will be matched to an existing character; if a character detection does not result in a match with a similarly higher than the threshold, it will be added as a new character to the visual coreference chains.
% We experiment with two methods to measure the similarity between two character crops: using features from pretrained CLIP ~\cite{radford2021learning,ilharco_gabriel_2021_5143773}, or using LVLMs~\cite{liu2024llavanext} to judge if two characters are the same character.
% Details of the two methods and the sequential matching algorithm are in the Appendix \ref{app:sequential_matching}.



\subsubsection{Textual Character Co-reference}
\label{sec:textual_coref}
Current state-of-the-art coreference resolution models generally struggle to effectively handle the coreference of plural nouns~\cite{liu2023detecting,le2023large,hicke2024lions}.
But plural nouns are very common in stories.
To address this issue,
we propose an LLM-based coreference resolution method (shown in Figure \ref{fig:coref_in_one}b).
Through in-context learning, this approach not only detects coreference relationships for singular characters but also identifies plural characters and all the singular characters they refer to.
More specifically, it consists of two steps:
\paragraph{Character Mention Detection} We propose a question-answering prompting method for LLMs to identify character mentions from all noun chunks and entities detected by spaCy, and mark these mentions with square brackets indicating a span to annotate in the next step (e.g., \textit{James $\rightarrow$ [James]}).
\paragraph{Character Co-reference Resolution} We propose a novel structured template prompt for LLMs to annotate these marked spans with cluster IDs (e.g., \textit{[James] $\rightarrow$ [James](\#1)}).
Note that there can be more than one cluster for plural characters (e.g., \textit{[We] $\rightarrow$ [We](\#1, \#2)}) to detect specific coreference relations for plural characters.
The prompts used in textual character coreference are shown in Appendix Table~\ref{tab:prompt_character_detection} and Table~\ref{tab:prompt_coreference_resolution}.

\subsubsection{Multimodal Character Alignment}
\label{sec:alignment}
At this stage, we aim to align textual coreference chains and visual coreference chains.
We model character alignment as a bipartite graph matching problem.
Specifically, we first generate a similarity matrix, where each element represents the similarity between each textual chain and each visual chain.
Then, we apply the Kuhn-Munkres algorithm to the similarity matrix and obtain the matching results.
Following \citet{liu2023detecting}, we employ the distributional similarity-based alignment algorithm to align the textual and visual chains. This method determines the alignment between textual and visual chains by comparing the distribution of characters in the images with their distribution in the sentences. For instance, textual mentions appearing first and second and visual appearances in the corresponding first and second images typically refer to the same character.

Mathematically, we employ a $C$-dimensional binary vector ($C$ is the number of images\footnote{In our experiments, we assume the number of sentences in a story is the same as the number of input images.}) to represent the distribution of a textual or visual character. More precisely, let $C_i$ denote the $i$-th textual character, then $C_i[k]=1$ means the $i$-th textual character is present in the $k$-th sentence. The representation for a visual character follows the same approach.
The similarity between a visual character and a textual character is computed as the dot product of their respective binary vectors.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../tacl_submission_2024"
%%% End: 

